African Languages AI Safety Readiness Report

With the widespread adoption of large language models (LLMs) across languages and domains, AI safety has emerged as a critical global concern. However, due to resource constraints, research and development efforts tend to prioritize a limited number of high-resource languages, leaving many others, especially those spoken in Africa, underrepresented. While existing research on language "resource-ness" has largely examined whether sufficient resources are available to develop language technologies, the question of whether languages are adequately represented in AI safety research has received attention only more recently. This report examines the readiness of African languages for inclusion in AI safety discussions, drawing on existing literature and data. It considers four factors: the availability of AI-relevant resources, including text data; national AI policy support; performance on established text benchmarks; and speaker population. Based on these factors, languages are grouped into four readiness categories: fully ready, mostly ready, emerging, and foundational support needed. This classification is intended to inform the inclusion of African languages in AI safety benchmarks, highlight varying levels of preparedness, and guide strategic investment in data development, policy, and community engagement for underrepresented languages.

==> tree.tex <==
  [Pretrained
    [{\textbf{Monolingual:} KinyaBERT~\cite{nzeyimana-niyongabo-rubungo-2022-kinyabert}, PuoBERTa~\cite{marivate2023puoberta}, OyoT5~\cite{olawole2024yadleveragingt5improved}, \\ SwahBERT~\cite{martin-etal-2022-swahbert},  EgyBERT~\cite{qarah2024egybert}, IgboBERT~\cite{chukwuneke-etal-2022-igbobert}}] 
    [{\textbf{Multilingual:} AfriBERTa(V2)~\cite{ogueji-etal-2021-small,oladipo2024scaling}, AfriTeVa(V2)~\cite{jude-ogundepo-etal-2022-afriteva,oladipo-etal-2023-better}, \\ Cheetah~\cite{adebara-etal-2024-cheetah}, Serengeti~\cite{adebara-etal-2023-serengeti}, InkubaLM~\cite{tonja2024inkubalmsmalllanguagemodel}, }] 
  ]
  [Adapted
    [{\textbf{Monolingual:} Amharic LLaMA~\cite{andersland2024amharicllamallavamultimodal}, Walia-LLM,}]
    [{\textbf{Multilingual:} AfroXLMR-\{76L, Social\}~\cite{alabi-etal-2022-adapting,adelani-etal-2024-sib,belay2025afroxlmrsocialadaptingpretrainedlanguage}, \\
    Nguni-XLMR~\cite{meyer-etal-2024-nglueni}}]  %
  ]

